Solving rough differential equations with the theory of regularity structures

The purpose of this article is to solve rough differential equations with the theory of regularity structures. These new tools recently developed by Martin Hairer for solving semi-linear partial differential stochastic equations were inspired by the rough path theory. We take a pedagogical approach to facilitate the understanding of this new theory. We recover results of the rough path theory with the regularity structure framework. Hence, we show how to formulate a fixed point problem in the abstract space of modelled distributions to solve the rough differential equations. We also give a proof of the existence of a rough path lift with the theory of regularity structure.

==> glossaire.tex <==
\newglossaryentry{est}
{
  name={$\est$},
  description={ratio of circumference of circle to its
               diameter},
  sort=pi
}
